Search for di-muon decays of a low-mass Higgs boson in radiative decays of the \Upsilon(1S)

We search for di-muon decays of a low-mass Higgs boson (A^0) produced in radiative \Upsilon(1S) decays. The \Upsilon(1S) sample is selected by tagging the pion pair in the \Upsilon(2S, 3S) \to \pi^+ \pi^- \Upsilon(1S) transitions, using a data sample of 92.8 \times 10^6 \Upsilon(2S) and 116.8 \times 10^6 \Upsilon(3S) events collected by the \babar\ detector. We find no evidence for A^0 production and set 90% confidence level upper limits on the product branching fraction \mathcal{B} (\Upsilon(1S) \to \gamma A^0) \times \mathcal{B} (A^0 \to \mumu) in the range of (0.28 - 9.7) \times 10^{-6} for 0.212 \le m_{A^0} \le 9.20 GeV/c^2. The results are combined with our previous measurements of \Upsilon(2S,3S) \to \gamma A^0, A^0 \to \mumu to set limits on the effective coupling of the \b-quark to the A^0.

==> ULYukawa.tex <==
HMass : Central value of the assumed A0 mass.
f_y :  90% C.L. upper limit on the effective Yukawa coupling (see Eq.(2) in the paper) of b-quark to the A0.  The combined result for this and the previous BABAR analysis PRL 103, 181801 (2009)] presented.
0.212	     2.8992e-07
0.214	     5.8972e-07
0.216	     9.2452e-07
0.218	     6.4882e-07
0.22	     6.5209e-07
0.222	     5.4669e-07
0.224	     5.028e-07
0.226	     6.1761e-07
0.228	     7.1405e-07
0.23	     6.88e-07
0.232	     5.6946e-07
0.234	     4.9984e-07
0.236	     4.7732e-07
0.238	     4.684e-07
0.24	     4.3739e-07
0.242	     4.1477e-07
0.244	     4.3013e-07
0.246	     4.3362e-07
0.248	     4.5166e-07
0.25	     4.2832e-07
0.252	     3.9798e-07
0.254	     3.8697e-07
0.256	     4.5487e-07
0.258	     4.8464e-07
0.26	     6.1963e-07
0.262	     5.9288e-07
0.264	     4.7497e-07
0.266	     4.1563e-07
0.268	     4.4479e-07
0.27	     4.6965e-07
0.272	     5.9716e-07
0.274	     5.9571e-07
0.276	     4.816e-07
0.278	     4.2823e-07
0.28	     4.6324e-07
0.282	     4.1271e-07
0.284	     4.4369e-07
0.286	     4.5756e-07
0.288	     4.8642e-07
0.29	     5.392e-07
0.292	     7.034e-07
0.294	     9.2563e-07
0.296	     9.2955e-07
0.298	     6.5245e-07
0.3	     4.9662e-07
0.302	     4.7186e-07
0.304	     4.6895e-07
0.306	     4.9662e-07
0.308	     5.4255e-07
0.31	     6.0099e-07
0.312	     5.709e-07
0.314	     5.4614e-07
0.316	     5.8001e-07
0.318	     5.9013e-07
0.32	     5.6451e-07
0.322	     5.1711e-07
0.324	     5.1202e-07
0.326	     5.4529e-07
0.328	     6.3352e-07
0.33	     6.9282e-07
0.332	     6.5358e-07
0.334	     5.829e-07
0.336	     5.4871e-07
0.338	     5.602e-07
0.34	     6.3116e-07
0.342	     7.0985e-07
0.344	     7.1691e-07
0.346	     7.4452e-07
0.348	     7.8189e-07
0.35	     1.0657e-06
0.352	     9.3846e-07
0.354	     1.1811e-06
0.356	     1.1773e-06
0.358	     1.0669e-06
0.36	     8.6254e-07
0.362	     7.7062e-07
0.364	     9.1082e-07
0.366	     9.3888e-07
0.368	     8.1593e-07
0.37	     8.8994e-07
0.372	     7.9178e-07
0.374	     9.431e-07
0.376	     6.9717e-07
0.378	     7.5179e-07
0.38	     7.2649e-07
0.382	     6.7586e-07
0.384	     5.8124e-07
0.386	     5.0747e-07
0.388	     4.8042e-07
0.39	     4.873e-07
0.392	     5.1071e-07
0.394	     5.5893e-07
0.396	     5.3434e-07
0.398	     5.5063e-07
0.4	     6.2708e-07
0.402	     7.9645e-07
0.404	     1.009e-06
0.406	     1.1216e-06
0.408	     1.0748e-06
0.41	     9.2689e-07
0.412	     7.5157e-07
0.414	     5.8983e-07
0.416	     5.0768e-07
0.418	     5.1551e-07
0.42	     6.1007e-07
0.422	     7.5607e-07
0.424	     8.5921e-07
0.426	     8.9747e-07
0.428	     9.2416e-07
0.43	     1.0104e-06
0.432	     1.1637e-06
0.434	     1.2807e-06
0.436	     1.1391e-06
0.438	     8.2119e-07
0.44	     6.0636e-07
0.442	     5.4943e-07
0.444	     5.4269e-07
0.446	     5.2272e-07
0.448	     4.7761e-07
0.45	     4.4046e-07
0.452	     4.3057e-07
0.454	     4.3057e-07
0.456	     4.2793e-07
0.458	     4.4842e-07
0.46	     5.1089e-07
0.462	     6.262e-07
0.464	     7.1805e-07
0.466	     6.9957e-07
0.468	     6.9164e-07
0.47	     7.8091e-07
0.472	     8.2452e-07
0.474	     7.5955e-07
0.476	     6.9466e-07
0.478	     7.0296e-07
0.48	     6.3283e-07
0.482	     7.4885e-07
0.484	     8.2879e-07
0.486	     6.3506e-07
0.488	     5.7146e-07
0.49	     6.8326e-07
0.492	     5.7409e-07
0.494	     5.0048e-07
0.496	     4.8349e-07
0.498	     4.6389e-07
0.5	     4.6875e-07
0.503	     4.6651e-07
0.506	     4.409e-07
0.509	     4.4266e-07
0.512	     4.6165e-07
0.515	     5.1871e-07
0.518	     6.0371e-07
0.521	     6.782e-07
0.524	     6.9388e-07
0.527	     6.599e-07
0.53	     6.2081e-07
0.533	     5.9212e-07
0.536	     5.4724e-07
0.539	     5.263e-07
0.542	     5.3714e-07
0.545	     5.4648e-07
0.548	     5.9192e-07
0.551	     6.6267e-07
0.554	     6.6716e-07
0.557	     6.0688e-07
0.56	     5.1839e-07
0.563	     4.738e-07
0.566	     4.7242e-07
0.569	     5.1328e-07
0.572	     5.618e-07
0.575	     5.6435e-07
0.578	     5.3626e-07
0.581	     5.2988e-07
0.584	     5.4137e-07
0.587	     5.8879e-07
0.59	     6.3032e-07
0.593	     6.2484e-07
0.596	     5.8124e-07
0.599	     5.4422e-07
0.602	     5.0125e-07
0.605	     4.4783e-07
0.608	     4.2594e-07
0.611	     4.3081e-07
0.614	     4.4176e-07
0.617	     4.4297e-07
0.62	     4.96e-07
0.623	     6.27e-07
0.626	     7.107e-07
0.629	     7.103e-07
0.632	     8.0192e-07
0.635	     8.5243e-07
0.638	     7.5826e-07
0.641	     6.9299e-07
0.644	     7.3837e-07
0.647	     8.7988e-07
0.65	     1.0569e-06
0.653	     1.4168e-06
0.656	     1.5121e-06
0.659	     1.5397e-06
0.662	     1.248e-06
0.665	     8.3434e-07
0.668	     6.4219e-07
0.671	     5.3028e-07
0.674	     5.9266e-07
0.677	     9.6506e-07
0.68	     9.2178e-07
0.683	     1.052e-06
0.686	     9.4026e-07
0.689	     8.1075e-07
0.692	     5.8853e-07
0.695	     4.9718e-07
0.698	     4.4665e-07
0.701	     4.4896e-07
0.704	     6.26e-07
0.707	     8.8933e-07
0.71	     1.1194e-06
0.713	     1.2089e-06
0.716	     1.1947e-06
0.719	     8.8672e-07
0.722	     7.3725e-07
0.725	     8.9392e-07
0.728	     1.0544e-06
0.731	     9.1212e-07
0.734	     7.9135e-07
0.737	     5.9089e-07
0.74	     4.9872e-07
0.743	     5.4269e-07
0.746	     6.3989e-07
0.749	     8.1332e-07
0.752	     8.2503e-07
0.755	     6.6187e-07
0.758	     5.013e-07
0.761	     4.7192e-07
0.764	     5.4129e-07
0.767	     7.6987e-07
0.77	     6.7181e-07
0.773	     5.6972e-07
0.776	     6.8943e-07
0.779	     9.4405e-07
0.782	     1.1131e-06
0.785	     1.0196e-06
0.788	     1.0199e-06
0.791	     1.1948e-06
0.794	     1.2116e-06
0.797	     9.0328e-07
0.8	     6.098e-07
0.803	     5.0359e-07
0.806	     4.6965e-07
0.809	     4.4577e-07
0.812	     4.3667e-07
0.815	     4.6055e-07
0.818	     5.0376e-07
0.821	     5.3902e-07
0.824	     5.6666e-07
0.827	     6.025e-07
0.83	     6.9785e-07
0.833	     8.0461e-07
0.836	     9.8826e-07
0.839	     1.2389e-06
0.842	     1.1076e-06
0.845	     9.0174e-07
0.848	     6.6809e-07
0.851	     5.9741e-07
0.854	     6.6802e-07
0.857	     8.1461e-07
0.86	     1.0604e-06
0.863	     1.5793e-06
0.866	     1.4343e-06
0.869	     7.7045e-07
0.872	     5.452e-07
0.875	     5.0933e-07
0.878	     5.9581e-07
0.881	     7.7397e-07
0.884	     8.7412e-07
0.887	     1.3719e-06
0.89	     1.4862e-06
0.893	     1.0489e-06
0.896	     8.4992e-07
0.899	     1.0169e-06
0.902	     1.3523e-06
0.905	     1.5347e-06
0.908	     1.3445e-06
0.911	     1.186e-06
0.914	     1.0269e-06
0.917	     9.7554e-07
0.92	     8.7183e-07
0.923	     5.9899e-07
0.926	     4.8048e-07
0.929	     4.4938e-07
0.932	     4.3246e-07
0.935	     4.1237e-07
0.938	     4.4621e-07
0.941	     5.0699e-07
0.944	     6.4467e-07
0.947	     6.6388e-07
0.95	     5.382e-07
0.953	     4.5255e-07
0.956	     4.4832e-07
0.959	     5.7606e-07
0.962	     8.11e-07
0.965	     7.9197e-07
0.968	     5.6992e-07
0.971	     5.0378e-07
0.974	     5.7423e-07
0.977	     6.178e-07
0.98	     5.8872e-07
0.983	     5.4648e-07
0.986	     5.7743e-07
0.989	     7.3698e-07
0.992	     6.8604e-07
0.995	     4.6476e-07
0.998	     4.0481e-07
1.001	     4.1206e-07
1.004	     4.1411e-07
1.007	     4.1512e-07
1.01	     4.1512e-07
1.013	     4.1919e-07
1.016	     4.8075e-07
1.019	     5.7798e-07
1.022	     7.1505e-07
1.025	     7.8195e-07
1.028	     9.4327e-07
1.031	     1.0793e-06
1.034	     9.1899e-07
1.037	     6.6609e-07
1.04	     6.1906e-07
1.043	     6.2998e-07
1.046	     6.7401e-07
1.049	     8.407e-07
1.05	     8.6402e-07
1.055	     9.0714e-07
1.06	     6.6494e-07
1.065	     6.6498e-07
1.07	     6.8736e-07
1.075	     8.1644e-07
1.08	     7.8725e-07
1.085	     9.1981e-07
1.09	     6.4507e-07
1.095	     5.6978e-07
1.1	     6.8272e-07
1.105	     1.0083e-06
1.11	     9.36e-07
1.115	     5.8504e-07
1.12	     4.8359e-07
1.125	     4.9776e-07
1.13	     5.5412e-07
1.135	     9.217e-07
1.14	     1.2231e-06
1.145	     1.3128e-06
1.15	     1.4667e-06
1.155	     1.36e-06
1.16	     8.6855e-07
1.165	     6.3694e-07
1.17	     8.5178e-07
1.175	     1.2092e-06
1.18	     1.0307e-06
1.185	     1.0847e-06
1.19	     1.1451e-06
1.195	     8.6903e-07
1.2	     9.6779e-07
1.205	     1.2835e-06
1.21	     1.3832e-06
1.215	     1.5131e-06
1.22	     1.5622e-06
1.225	     1.1183e-06
1.23	     8.5732e-07
1.235	     1.2539e-06
1.24	     1.3035e-06
1.245	     9.8315e-07
1.25	     7.1858e-07
1.255	     7.0344e-07
1.26	     7.7088e-07
1.265	     7.8907e-07
1.27	     1.1912e-06
1.275	     1.0943e-06
1.28	     7.8482e-07
1.285	     7.2875e-07
1.29	     7.5472e-07
1.295	     1.0103e-06
1.3	     9.9856e-07
1.305	     9.2695e-07
1.31	     9.1825e-07
1.315	     9.0853e-07
1.32	     9.7673e-07
1.325	     1.055e-06
1.33	     1.2858e-06
1.335	     1.3925e-06
1.34	     1.26e-06
1.345	     9.113e-07
1.35	     9.961e-07
1.355	     7.003e-07
1.36	     4.1839e-07
1.365	     4.1297e-07
1.37	     5.4641e-07
1.375	     6.0838e-07
1.38	     6.6667e-07
1.385	     8.4348e-07
1.39	     8.3203e-07
1.395	     9.211e-07
1.4	     8.1402e-07
1.405	     7.4484e-07
1.41	     1.0591e-06
1.415	     1.1165e-06
1.42	     1.0623e-06
1.425	     8.4765e-07
1.43	     5.9823e-07
1.435	     6.0949e-07
1.44	     8.0152e-07
1.445	     8.9243e-07
1.45	     7.5514e-07
1.455	     6.4453e-07
1.46	     6.7873e-07
1.465	     7.6888e-07
1.47	     8.4434e-07
1.475	     8.5316e-07
1.48	     8.7571e-07
1.485	     9.1787e-07
1.49	     7.3245e-07
1.495	     6.6899e-07
1.5	     7.3384e-07
1.505	     8.1322e-07
1.51	     6.6524e-07
1.515	     7.0512e-07
1.52	     1.3407e-06
1.525	     1.4882e-06
1.53	     9.4067e-07
1.535	     7.4122e-07
1.54	     1.1069e-06
1.545	     1.268e-06
1.55	     9.583e-07
1.555	     1.1218e-06
1.56	     1.1638e-06
1.565	     8.834e-07
1.57	     8.8442e-07
1.575	     7.9677e-07
1.58	     7.1896e-07
1.585	     8.072e-07
1.59	     7.1438e-07
1.595	     4.8655e-07
1.6	     4.3721e-07
1.605	     4.8569e-07
1.61	     4.8927e-07
1.615	     6.6537e-07
1.62	     1.0444e-06
1.625	     1.6034e-06
1.63	     1.5291e-06
1.635	     9.2172e-07
1.64	     9.3264e-07
1.645	     9.2506e-07
1.65	     8.8142e-07
1.655	     6.2944e-07
1.66	     4.4242e-07
1.665	     4.1396e-07
1.67	     3.924e-07
1.675	     4.6055e-07
1.68	     5.9888e-07
1.685	     7.3322e-07
1.69	     1.089e-06
1.695	     8.767e-07
1.7	     9.0592e-07
1.705	     1.5354e-06
1.71	     1.5258e-06
1.715	     1.2328e-06
1.72	     9.392e-07
1.725	     1.094e-06
1.73	     1.3672e-06
1.735	     1.2548e-06
1.74	     1.0385e-06
1.745	     8.7719e-07
1.75	     7.9289e-07
1.755	     7.0299e-07
1.76	     5.5127e-07
1.765	     4.721e-07
1.77	     5.9077e-07
1.775	     5.6092e-07
1.78	     4.2749e-07
1.785	     4.3324e-07
1.79	     5.9215e-07
1.795	     6.9882e-07
1.8	     9.6858e-07
1.805	     1.0813e-06
1.81	     9.304e-07
1.815	     6.7827e-07
1.82	     4.9272e-07
1.825	     5.451e-07
1.83	     8.2602e-07
1.835	     1.0762e-06
1.84	     9.4141e-07
1.845	     7.6704e-07
1.85	     6.7229e-07
1.855	     5.6463e-07
1.86	     5.2024e-07
1.865	     7.8835e-07
1.87	     1.0567e-06
1.875	     1.1881e-06
1.88	     1.1511e-06
1.885	     6.9958e-07
1.89	     6.3265e-07
1.895	     5.5108e-07
1.9	     4.8806e-07
1.905	     5.5214e-07
1.91	     5.5751e-07
1.915	     7.4689e-07
1.92	     9.3641e-07
1.925	     7.631e-07
1.93	     6.7738e-07
1.935	     8.234e-07
1.94	     7.3385e-07
1.945	     5.6286e-07
1.95	     8.2292e-07
1.955	     1.2312e-06
1.96	     1.2233e-06
1.965	     1.0566e-06
1.97	     8.6241e-07
1.975	     8.7352e-07
1.98	     9.6503e-07
1.985	     7.6721e-07
1.99	     6.4908e-07
1.995	     9.069e-07
2	     9.0466e-07
2.005	     6.7022e-07
2.01	     5.9947e-07
2.015	     6.4897e-07
2.02	     6.6538e-07
2.025	     6.9259e-07
2.03	     7.6721e-07
2.035	     6.2325e-07
2.04	     5.2493e-07
2.045	     5.3371e-07
2.05	     5.5281e-07
2.055	     5.4688e-07
2.06	     6.5013e-07
2.065	     8.3635e-07
2.07	     7.2331e-07
2.075	     6.5974e-07
2.08	     1.0848e-06
2.085	     1.4459e-06
2.09	     1.4061e-06
2.095	     1.1393e-06
2.1	     1.0792e-06
2.105	     1.1347e-06
2.11	     8.7732e-07
2.115	     5.6907e-07
2.12	     5.2756e-07
2.125	     5.7451e-07
2.13	     4.8078e-07
2.135	     4.5981e-07
2.14	     4.7869e-07
2.145	     4.5362e-07
2.15	     4.5209e-07
2.155	     5.7233e-07
2.16	     8.7299e-07
2.165	     9.1243e-07
2.17	     1.016e-06
2.175	     1.2692e-06
2.18	     1.5179e-06
2.185	     1.6157e-06
2.19	     1.3843e-06
2.195	     1.1455e-06
2.2	     1.002e-06
2.205	     1.1203e-06
2.21	     1.2077e-06
2.215	     9.4247e-07
2.22	     6.6977e-07
2.225	     6.2325e-07
2.23	     5.5628e-07
2.235	     6.5874e-07
2.24	     8.936e-07
2.245	     7.8208e-07
2.25	     6.2588e-07
2.255	     6.7778e-07
2.26	     6.5522e-07
2.265	     6.3092e-07
2.27	     7.1103e-07
2.275	     9.6325e-07
2.28	     1.274e-06
2.285	     1.4884e-06
2.29	     1.4591e-06
2.295	     1.0124e-06
2.3	     5.2157e-07
2.305	     4.3065e-07
2.31	     5.3187e-07
2.315	     1.0411e-06
2.32	     1.4472e-06
2.325	     1.245e-06
2.33	     9.0554e-07
2.335	     5.9867e-07
2.34	     4.7753e-07
2.345	     5.1264e-07
2.35	     5.5753e-07
2.355	     5.9073e-07
2.36	     6.8363e-07
2.365	     7.4175e-07
2.37	     8.2475e-07
2.375	     1.0462e-06
2.38	     1.3828e-06
2.385	     1.4044e-06
2.39	     1.487e-06
2.395	     1.7683e-06
2.4	     1.6958e-06
2.405	     1.1512e-06
2.41	     8.1543e-07
2.415	     6.2018e-07
2.42	     5.5123e-07
2.425	     9.0609e-07
2.43	     1.2287e-06
2.435	     8.8783e-07
2.44	     7.5812e-07
2.445	     9.0897e-07
2.45	     9.9772e-07
2.455	     9.7834e-07
2.46	     1.0582e-06
2.465	     9.6592e-07
2.47	     8.6816e-07
2.475	     1.02e-06
2.48	     1.0553e-06
2.485	     8.7738e-07
2.49	     6.5608e-07
2.495	     7.1015e-07
2.5	     7.7379e-07
2.505	     7.6223e-07
2.51	     7.7788e-07
2.515	     8.5049e-07
2.52	     9.9151e-07
2.525	     9.2389e-07
2.53	     7.2799e-07
2.535	     6.9869e-07
2.54	     8.4517e-07
2.545	     1.2749e-06
2.55	     1.2272e-06
2.555	     7.0989e-07
2.56	     4.6776e-07
2.565	     4.7314e-07
2.57	     6.8182e-07
2.575	     7.8876e-07
2.58	     7.1384e-07
2.585	     6.7781e-07
2.59	     7.1467e-07
2.595	     7.8392e-07
2.6	     8.1144e-07
2.605	     8.3216e-07
2.61	     8.0896e-07
2.615	     6.0565e-07
2.62	     5.1386e-07
2.625	     7.5906e-07
2.63	     1.4725e-06
2.635	     2.1139e-06
2.64	     2.0175e-06
2.645	     1.2519e-06
2.65	     8.887e-07
2.655	     1.0767e-06
2.66	     1.59e-06
2.665	     1.6787e-06
2.67	     1.2884e-06
2.675	     8.7643e-07
2.68	     5.9457e-07
2.685	     5.1048e-07
2.69	     5.2468e-07
2.695	     5.8354e-07
2.7	     8.692e-07
2.705	     1.3457e-06
2.71	     1.6465e-06
2.715	     1.4821e-06
2.72	     1.0473e-06
2.725	     7.6752e-07
2.73	     7.3769e-07
2.735	     7.3398e-07
2.74	     8.3787e-07
2.745	     1.095e-06
2.75	     1.0229e-06
2.755	     8.6357e-07
2.76	     9.6819e-07
2.765	     1.0912e-06
2.77	     1.1224e-06
2.775	     1.2027e-06
2.78	     1.1265e-06
2.785	     9.4714e-07
2.79	     7.227e-07
2.795	     5.9548e-07
2.8	     9.0229e-07
2.805	     1.3694e-06
2.81	     1.2819e-06
2.815	     1.081e-06
2.82	     9.0229e-07
2.825	     7.5861e-07
2.83	     9.3315e-07
2.835	     1.3253e-06
2.84	     1.6157e-06
2.845	     1.8681e-06
2.85	     1.7034e-06
2.855	     1.1303e-06
2.86	     7.398e-07
2.865	     6.3995e-07
2.87	     8.0024e-07
2.875	     9.7299e-07
2.88	     9.0183e-07
2.885	     1.011e-06
2.89	     1.2467e-06
2.895	     1.4122e-06
2.9	     1.1114e-06
2.905	     7.0845e-07
2.91	     5.5931e-07
2.915	     5.9165e-07
2.92	     6.4519e-07
2.925	     7.3509e-07
2.93	     9.9203e-07
2.935	     1.2392e-06
2.94	     1.4118e-06
2.945	     1.6447e-06
2.95	     1.8441e-06
2.955	     1.8927e-06
2.96	     1.8381e-06
2.965	     1.7118e-06
2.97	     1.3105e-06
2.975	     8.3452e-07
2.98	     6.1616e-07
2.985	     5.6104e-07
2.99	     5.3959e-07
2.995	     4.9033e-07
3	     5.2932e-07
3.005	     6.1622e-07
3.01	     7.3122e-07
3.015	     7.2532e-07
3.02	     6.6495e-07
3.025	     6.5696e-07
3.03	     5.6552e-07
3.035	     6.5985e-07
3.04	     8.807e-07
3.045	     1.7683e-06
3.05	     1.2032e-06
3.055	     1.0688e-06
3.06	     1.188e-06
3.065	     1.5942e-06
3.07	     2.0512e-06
3.075	     2.0555e-06
3.08	     2.0091e-06
3.085	     2.7496e-06
3.09	     3.8753e-06
3.095	     4.5032e-06
3.1	     4.1056e-06
3.105	     3.1311e-06
3.11	     2.4867e-06
3.115	     2.7258e-06
3.12	     3.2251e-06
3.125	     3.3178e-06
3.13	     2.7628e-06
3.135	     1.781e-06
3.14	     1.4271e-06
3.145	     1.4274e-06
3.15	     1.4708e-06
3.155	     1.7983e-06
3.16	     2.2513e-06
3.165	     1.3922e-06
3.17	     1.3904e-06
3.175	     1.0414e-06
3.18	     8.5347e-07
3.185	     1.0122e-06
3.19	     1.5315e-06
3.195	     2.0211e-06
3.2	     1.9318e-06
3.205	     1.4958e-06
3.21	     1.2138e-06
3.215	     1.1278e-06
3.22	     1.1829e-06
3.225	     1.2526e-06
3.23	     1.0792e-06
3.235	     9.7001e-07
3.24	     9.3827e-07
3.245	     7.1123e-07
3.25	     5.7914e-07
3.255	     5.7097e-07
3.26	     5.6824e-07
3.265	     5.51e-07
3.27	     5.4879e-07
3.275	     6.4381e-07
3.28	     9.5454e-07
3.285	     1.4478e-06
3.29	     1.9275e-06
3.295	     1.8651e-06
3.3	     1.3349e-06
3.305	     1.1191e-06
3.31	     1.3125e-06
3.315	     1.3802e-06
3.32	     1.2583e-06
3.325	     1.2992e-06
3.33	     1.3344e-06
3.335	     1.3449e-06
3.34	     1.5085e-06
3.345	     1.4276e-06
3.35	     1.2246e-06
3.355	     1.0939e-06
3.36	     9.4146e-07
3.365	     1.0404e-06
3.37	     1.2994e-06
3.375	     1.296e-06
3.38	     1.1415e-06
3.385	     1.1319e-06
3.39	     1.1163e-06
3.395	     1.0557e-06
3.4	     1.0808e-06
3.405	     1.1437e-06
3.41	     1.1789e-06
3.415	     1.1447e-06
3.42	     1.1222e-06
3.425	     1.0779e-06
3.43	     8.2163e-07
3.435	     6.0138e-07
3.44	     6.1345e-07
3.445	     7.84e-07
3.45	     9.6847e-07
3.455	     9.9795e-07
3.46	     9.5318e-07
3.465	     8.8325e-07
3.47	     8.3052e-07
3.475	     9.5692e-07
3.48	     1.3824e-06
3.485	     1.7124e-06
3.49	     2.0665e-06
3.495	     2.5113e-06
3.5	     2.1556e-06
3.505	     1.2304e-06
3.51	     8.7198e-07
3.515	     9.0663e-07
3.52	     9.557e-07
3.525	     9.6431e-07
3.53	     8.3793e-07
3.535	     8.3348e-07
3.54	     1.1631e-06
3.545	     1.7083e-06
3.55	     1.7893e-06
3.555	     1.353e-06
3.56	     1.3013e-06
3.565	     1.5114e-06
3.57	     1.6672e-06
3.575	     1.8753e-06
3.58	     2.2265e-06
3.585	     2.4309e-06
3.59	     2.1244e-06
3.595	     1.4635e-06
3.6	     1.0237e-06
3.605	     7.7184e-07
3.61	     6.5387e-07
3.615	     7.5337e-07
3.62	     9.6372e-07
3.625	     1.3475e-06
3.63	     1.9106e-06
3.635	     1.9723e-06
3.64	     1.3607e-06
3.645	     9.059e-07
3.65	     6.7793e-07
3.655	     5.2697e-07
3.66	     1.036e-06
3.665	     1.3129e-06
3.67	     1.7264e-06
3.675	     1.9186e-06
3.68	     2.341e-06
3.685	     2.8453e-06
3.69	     2.8815e-06
3.695	     2.5528e-06
3.7	     2.446e-06
3.705	     2.3617e-06
3.71	     1.3493e-06
3.715	     1.3202e-06
3.72	     1.5263e-06
3.725	     1.7211e-06
3.73	     1.6478e-06
3.735	     1.653e-06
3.74	     1.989e-06
3.745	     2.1809e-06
3.75	     1.8798e-06
3.755	     1.4297e-06
3.76	     1.3078e-06
3.765	     1.4914e-06
3.77	     1.6805e-06
3.775	     1.7223e-06
3.78	     1.699e-06
3.785	     1.5485e-06
3.79	     1.2767e-06
3.795	     1.0128e-06
3.8	     9.1446e-07
3.805	     9.2469e-07
3.81	     1.0714e-06
3.815	     1.2556e-06
3.82	     1.2735e-06
3.825	     1.2533e-06
3.83	     1.3446e-06
3.835	     1.481e-06
3.84	     1.5413e-06
3.845	     1.5093e-06
3.85	     1.3188e-06
3.855	     9.9941e-07
3.86	     8.0753e-07
3.865	     8.1906e-07
3.87	     9.1368e-07
3.875	     1.0541e-06
3.88	     1.2255e-06
3.885	     1.0965e-06
3.89	     8.5737e-07
3.895	     8.1808e-07
3.9	     8.8519e-07
3.905	     9.3403e-07
3.91	     8.2715e-07
3.915	     6.6494e-07
3.92	     6.8529e-07
3.925	     9.8331e-07
3.93	     1.3634e-06
3.935	     1.4275e-06
3.94	     1.3275e-06
3.945	     1.2925e-06
3.95	     1.3472e-06
3.955	     1.5312e-06
3.96	     1.6588e-06
3.965	     1.6496e-06
3.97	     1.6625e-06
3.975	     1.6315e-06
3.98	     1.456e-06
3.985	     1.3853e-06
3.99	     1.3541e-06
3.995	     1.1578e-06
4	     9.1991e-07
4.005	     9.1437e-07
4.01	     9.2694e-07
4.015	     8.8085e-07
4.02	     9.3682e-07
4.025	     9.6808e-07
4.03	     9.5665e-07
4.035	     1.1355e-06
4.04	     1.5807e-06
4.045	     1.6881e-06
4.05	     1.3757e-06
4.055	     1.0353e-06
4.06	     9.4268e-07
4.065	     1.0929e-06
4.07	     1.3459e-06
4.075	     1.444e-06
4.08	     1.3899e-06
4.085	     1.19e-06
4.09	     9.9852e-07
4.095	     8.4265e-07
4.1	     7.3688e-07
4.105	     8.2845e-07
4.11	     1.1592e-06
4.115	     1.6897e-06
4.12	     2.1591e-06
4.125	     2.0617e-06
4.13	     1.6305e-06
4.135	     1.3469e-06
4.14	     1.7341e-06
4.145	     2.611e-06
4.15	     2.9855e-06
4.155	     2.5197e-06
4.16	     1.9406e-06
4.165	     1.7402e-06
4.17	     1.446e-06
4.175	     1.1971e-06
4.18	     1.196e-06
4.185	     1.2678e-06
4.19	     1.2871e-06
4.195	     1.1199e-06
4.2	     7.7959e-07
4.205	     6.3641e-07
4.21	     7.2419e-07
4.215	     1.0281e-06
4.22	     1.4593e-06
4.225	     1.7786e-06
4.23	     1.7697e-06
4.235	     1.4714e-06
4.24	     1.4992e-06
4.245	     2.023e-06
4.25	     2.5616e-06
4.255	     2.2434e-06
4.26	     1.5798e-06
4.265	     1.1881e-06
4.27	     9.7756e-07
4.275	     9.2091e-07
4.28	     1.1667e-06
4.285	     1.5942e-06
4.29	     1.619e-06
4.295	     1.5273e-06
4.3	     1.6626e-06
4.305	     1.6512e-06
4.31	     1.5067e-06
4.315	     1.2475e-06
4.32	     1.1065e-06
4.325	     1.1292e-06
4.33	     1.1356e-06
4.335	     1.1486e-06
4.34	     1.068e-06
4.345	     9.6735e-07
4.35	     1.135e-06
4.355	     1.2936e-06
4.36	     1.3175e-06
4.365	     1.4641e-06
4.37	     1.7518e-06
4.375	     1.699e-06
4.38	     1.2864e-06
4.385	     9.636e-07
4.39	     9.0518e-07
4.395	     9.5786e-07
4.4	     1.0692e-06
4.405	     1.1018e-06
4.41	     1.0119e-06
4.415	     9.4301e-07
4.42	     1.0609e-06
4.425	     1.4773e-06
4.43	     1.8186e-06
4.435	     1.515e-06
4.44	     1.0738e-06
4.445	     8.3775e-07
4.45	     8.0414e-07
4.455	     8.9821e-07
4.46	     1.2046e-06
4.465	     2.0671e-06
4.47	     2.9757e-06
4.475	     3.4224e-06
4.48	     3.4133e-06
4.485	     3.1983e-06
4.49	     2.8816e-06
4.495	     2.5251e-06
4.5	     2.8082e-06
4.505	     3.4979e-06
4.51	     3.3509e-06
4.515	     2.2225e-06
4.52	     1.3948e-06
4.525	     1.2219e-06
4.53	     1.2882e-06
4.535	     1.1974e-06
4.54	     8.8926e-07
4.545	     7.4825e-07
4.55	     8.9018e-07
4.555	     1.2844e-06
4.56	     1.5471e-06
4.565	     1.5522e-06
4.57	     1.6456e-06
4.575	     1.655e-06
4.58	     1.4808e-06
4.585	     1.4126e-06
4.59	     1.5064e-06
4.595	     1.5596e-06
4.6	     1.323e-06
4.605	     9.7569e-07
4.61	     8.6396e-07
4.615	     9.3812e-07
4.62	     1.0244e-06
4.625	     9.6981e-07
4.63	     9.9233e-07
4.635	     1.203e-06
4.64	     1.3438e-06
4.645	     1.4627e-06
4.65	     1.7936e-06
4.655	     1.8398e-06
4.66	     1.3277e-06
4.665	     1.0778e-06
4.67	     1.3156e-06
4.675	     1.6052e-06
4.68	     1.5546e-06
4.685	     1.4798e-06
4.69	     1.6934e-06
4.695	     1.6608e-06
4.7	     1.3691e-06
4.705	     1.1914e-06
4.71	     1.4318e-06
4.715	     1.7536e-06
4.72	     1.9803e-06
4.725	     1.749e-06
4.73	     1.4096e-06
4.735	     1.0785e-06
4.74	     9.7844e-07
4.745	     1.0754e-06
4.75	     1.0078e-06
4.755	     8.1293e-07
4.76	     7.6684e-07
4.765	     9.0418e-07
4.77	     1.194e-06
4.775	     1.4729e-06
4.78	     1.6539e-06
4.785	     1.9326e-06
4.79	     2.0799e-06
4.795	     2.0426e-06
4.8	     1.7734e-06
4.805	     1.5225e-06
4.81	     1.4659e-06
4.815	     1.5481e-06
4.82	     1.7759e-06
4.825	     1.7998e-06
4.83	     1.9355e-06
4.835	     2.0117e-06
4.84	     1.6722e-06
4.845	     1.2162e-06
4.85	     1.204e-06
4.855	     1.6541e-06
4.86	     2.076e-06
4.865	     1.5462e-06
4.87	     1.167e-06
4.875	     1.0477e-06
4.88	     9.9954e-07
4.885	     9.6017e-07
4.89	     9.7038e-07
4.895	     1.0938e-06
4.9	     1.2968e-06
4.905	     1.3979e-06
4.91	     1.3844e-06
4.915	     1.2783e-06
4.92	     1.145e-06
4.925	     1.1643e-06
4.93	     1.4905e-06
4.935	     2.5209e-06
4.94	     3.057e-06
4.945	     2.3796e-06
4.95	     1.6182e-06
4.955	     1.3486e-06
4.96	     1.3084e-06
4.965	     1.4257e-06
4.97	     1.645e-06
4.975	     2.002e-06
4.98	     2.1987e-06
4.985	     2.0358e-06
4.99	     1.8288e-06
4.995	     1.8903e-06
5	     2.0281e-06
5.005	     2.0396e-06
5.01	     1.8861e-06
5.015	     1.6409e-06
5.02	     1.3661e-06
5.025	     1.4142e-06
5.03	     1.8486e-06
5.035	     2.4971e-06
5.04	     2.9841e-06
5.045	     2.9084e-06
5.05	     2.0426e-06
5.055	     1.2738e-06
5.06	     1.1542e-06
5.065	     1.3211e-06
5.07	     1.4283e-06
5.075	     1.2825e-06
5.08	     1.0281e-06
5.085	     8.3899e-07
5.09	     7.6564e-07
5.095	     8.5068e-07
5.1	     1.1382e-06
5.105	     1.4766e-06
5.11	     1.4563e-06
5.115	     1.3214e-06
5.12	     1.3434e-06
5.125	     1.519e-06
5.13	     1.9795e-06
5.135	     2.5173e-06
5.14	     2.7802e-06
5.145	     3.1176e-06
5.15	     3.445e-06
5.155	     3.2375e-06
5.16	     2.4858e-06
5.165	     1.6161e-06
5.17	     1.1425e-06
5.175	     1.0704e-06
5.18	     1.2576e-06
5.185	     1.4339e-06
5.19	     1.547e-06
5.195	     2.0057e-06
5.2	     3.0704e-06
5.205	     4.2263e-06
5.21	     4.5338e-06
5.215	     3.141e-06
5.22	     1.8684e-06
5.225	     1.113e-06
5.23	     1.0205e-06
5.235	     1.199e-06
5.24	     1.4248e-06
5.245	     1.5515e-06
5.25	     1.7775e-06
5.255	     1.9286e-06
5.26	     1.9565e-06
5.265	     1.782e-06
5.27	     1.7806e-06
5.275	     2.0459e-06
5.28	     1.7414e-06
5.285	     1.3475e-06
5.29	     1.1288e-06
5.295	     1.1015e-06
5.3	     1.2451e-06
5.305	     1.5457e-06
5.31	     1.936e-06
5.315	     2.4313e-06
5.32	     2.8329e-06
5.325	     2.7228e-06
5.33	     1.9868e-06
5.335	     1.5025e-06
5.34	     1.3474e-06
5.345	     1.4709e-06
5.35	     1.6315e-06
5.355	     1.6476e-06
5.36	     1.458e-06
5.365	     1.6952e-06
5.37	     2.1537e-06
5.375	     2.9708e-06
5.38	     3.3168e-06
5.385	     2.8271e-06
5.39	     2.1251e-06
5.395	     1.9451e-06
5.4	     2.1145e-06
5.405	     2.3488e-06
5.41	     2.472e-06
5.415	     1.8989e-06
5.42	     1.4497e-06
5.425	     1.3821e-06
5.43	     1.4913e-06
5.435	     1.6218e-06
5.44	     1.7757e-06
5.445	     1.8985e-06
5.45	     1.9369e-06
5.455	     2.2809e-06
5.46	     2.7883e-06
5.465	     3.1255e-06
5.47	     3.1005e-06
5.475	     2.7557e-06
5.48	     2.112e-06
5.485	     1.8653e-06
5.49	     1.7925e-06
5.495	     1.9736e-06
5.5	     2.3963e-06
5.505	     2.5493e-06
5.51	     2.3974e-06
5.515	     2.062e-06
5.52	     1.4259e-06
5.525	     1.0689e-06
5.53	     1.0733e-06
5.535	     1.1545e-06
5.54	     1.2449e-06
5.545	     1.4355e-06
5.55	     1.6512e-06
5.555	     1.6269e-06
5.56	     2.0558e-06
5.565	     2.8964e-06
5.57	     3.6366e-06
5.575	     3.5556e-06
5.58	     2.8924e-06
5.585	     2.1491e-06
5.59	     1.6544e-06
5.595	     1.1736e-06
5.6	     9.2186e-07
5.605	     8.7486e-07
5.61	     9.2614e-07
5.615	     1.1636e-06
5.62	     1.8388e-06
5.625	     2.4974e-06
5.63	     2.2192e-06
5.635	     1.7053e-06
5.64	     1.5493e-06
5.645	     1.7226e-06
5.65	     2.019e-06
5.655	     2.1428e-06
5.66	     2.4148e-06
5.665	     2.8282e-06
5.67	     3.1426e-06
5.675	     3.1742e-06
5.68	     3.0706e-06
5.685	     3.5862e-06
5.69	     4.0658e-06
5.695	     4.4985e-06
5.7	     4.4011e-06
5.705	     3.9035e-06
5.71	     2.9723e-06
5.715	     2.35e-06
5.72	     2.3446e-06
5.725	     2.5057e-06
5.73	     2.447e-06
5.735	     2.3996e-06
5.74	     2.3687e-06
5.745	     2.4114e-06
5.75	     2.3443e-06
5.755	     2.2154e-06
5.76	     2.3043e-06
5.765	     2.4588e-06
5.77	     2.3116e-06
5.775	     2.3182e-06
5.78	     2.3667e-06
5.785	     2.2189e-06
5.79	     1.8902e-06
5.795	     1.6889e-06
5.8	     1.7023e-06
5.805	     1.7885e-06
5.81	     1.7222e-06
5.815	     1.4743e-06
5.82	     1.366e-06
5.825	     1.5068e-06
5.83	     1.5392e-06
5.835	     1.5626e-06
5.84	     1.5736e-06
5.845	     1.5476e-06
5.85	     1.8151e-06
5.855	     2.2824e-06
5.86	     2.4546e-06
5.865	     2.2272e-06
5.87	     1.9859e-06
5.875	     1.9423e-06
5.88	     2.1182e-06
5.885	     2.1275e-06
5.89	     1.9429e-06
5.895	     1.9902e-06
5.9	     2.434e-06
5.905	     3.2202e-06
5.91	     3.7702e-06
5.915	     3.8774e-06
5.92	     4.1574e-06
5.925	     5.1599e-06
5.93	     5.913e-06
5.935	     5.0935e-06
5.94	     3.5734e-06
5.945	     2.4747e-06
5.95	     1.7638e-06
5.955	     1.4978e-06
5.96	     1.5493e-06
5.965	     1.9604e-06
5.97	     2.3727e-06
5.975	     2.5444e-06
5.98	     2.3043e-06
5.985	     1.9446e-06
5.99	     1.6194e-06
5.995	     1.3875e-06
6	     1.2722e-06
6.005	     1.2115e-06
6.01	     1.318e-06
6.015	     1.4782e-06
6.02	     1.7285e-06
6.025	     2.154e-06
6.03	     2.3288e-06
6.035	     2.3189e-06
6.04	     2.3118e-06
6.045	     2.6069e-06
6.05	     3.006e-06
6.055	     2.9883e-06
6.06	     2.5299e-06
6.065	     2.1498e-06
6.07	     1.8713e-06
6.075	     1.6626e-06
6.08	     1.7062e-06
6.085	     1.7556e-06
6.09	     1.8027e-06
6.095	     1.681e-06
6.1	     1.6412e-06
6.105	     1.7602e-06
6.11	     2.0336e-06
6.115	     2.1249e-06
6.12	     2.0875e-06
6.125	     2.233e-06
6.13	     2.9564e-06
6.135	     3.6396e-06
6.14	     3.7578e-06
6.145	     2.936e-06
6.15	     2.1694e-06
6.155	     1.8294e-06
6.16	     1.9277e-06
6.165	     2.1247e-06
6.17	     2.344e-06
6.175	     2.4258e-06
6.18	     2.4569e-06
6.185	     2.3179e-06
6.19	     2.436e-06
6.195	     2.4248e-06
6.2	     2.3742e-06
6.205	     2.0814e-06
6.21	     1.9023e-06
6.215	     2.3267e-06
6.22	     3.1107e-06
6.225	     3.7692e-06
6.23	     4.2347e-06
6.235	     4.6473e-06
6.24	     4.703e-06
6.245	     4.6658e-06
6.25	     4.8048e-06
6.255	     4.3478e-06
6.26	     3.5588e-06
6.265	     3.2379e-06
6.27	     2.6464e-06
6.275	     2.1072e-06
6.28	     1.863e-06
6.285	     1.8346e-06
6.29	     1.8839e-06
6.295	     1.7033e-06
6.3	     1.6328e-06
6.305	     1.5987e-06
6.31	     1.3039e-06
6.315	     1.1877e-06
6.32	     1.3065e-06
6.325	     1.4272e-06
6.33	     1.4461e-06
6.335	     1.5169e-06
6.34	     1.7339e-06
6.345	     2.1479e-06
6.35	     2.9157e-06
6.355	     3.8982e-06
6.36	     4.7057e-06
6.365	     4.4422e-06
6.37	     3.6293e-06
6.375	     2.9313e-06
6.38	     2.7013e-06
6.385	     2.3461e-06
6.39	     2.1594e-06
6.395	     2.2657e-06
6.4	     2.5207e-06
6.405	     2.6312e-06
6.41	     2.6784e-06
6.415	     2.3813e-06
6.42	     2.1323e-06
6.425	     2.1707e-06
6.43	     2.3631e-06
6.435	     2.6434e-06
6.44	     2.9537e-06
6.445	     3.6071e-06
6.45	     4.7107e-06
6.455	     4.8239e-06
6.46	     4.5849e-06
6.465	     4.5084e-06
6.47	     4.3998e-06
6.475	     4.2578e-06
6.48	     3.7505e-06
6.485	     3.6016e-06
6.49	     3.3467e-06
6.495	     2.9546e-06
6.5	     2.8093e-06
6.505	     3.1355e-06
6.51	     3.3773e-06
6.515	     3.2223e-06
6.52	     3.1005e-06
6.525	     3.5655e-06
6.53	     3.8151e-06
6.535	     3.4648e-06
6.54	     2.5831e-06
6.545	     2.0973e-06
6.55	     2.1932e-06
6.555	     2.3964e-06
6.56	     2.3742e-06
6.565	     2.1438e-06
6.57	     1.934e-06
6.575	     2.1983e-06
6.58	     2.7878e-06
6.585	     3.2276e-06
6.59	     2.954e-06
6.595	     2.5856e-06
6.6	     2.6722e-06
6.605	     2.8075e-06
6.61	     2.6416e-06
6.615	     2.6573e-06
6.62	     2.711e-06
6.625	     3.1995e-06
6.63	     3.4638e-06
6.635	     3.3423e-06
6.64	     3.538e-06
6.645	     3.631e-06
6.65	     3.6839e-06
6.655	     3.5099e-06
6.66	     3.1999e-06
6.665	     3.1498e-06
6.67	     3.3852e-06
6.675	     3.9306e-06
6.68	     4.4236e-06
6.685	     4.3521e-06
6.69	     3.8162e-06
6.695	     3.1899e-06
6.7	     2.7965e-06
6.705	     2.7112e-06
6.71	     2.7706e-06
6.715	     2.9006e-06
6.72	     2.9293e-06
6.725	     3.1362e-06
6.73	     3.6638e-06
6.735	     3.7914e-06
6.74	     3.4962e-06
6.745	     3.4309e-06
6.75	     4.0096e-06
6.755	     4.0587e-06
6.76	     3.1242e-06
6.765	     2.4762e-06
6.77	     2.4207e-06
6.775	     2.9114e-06
6.78	     4.4415e-06
6.785	     6.0479e-06
6.79	     5.9173e-06
6.795	     4.6097e-06
6.8	     3.5149e-06
6.805	     3.2891e-06
6.81	     3.915e-06
6.815	     4.9711e-06
6.82	     5.2185e-06
6.825	     5.0451e-06
6.83	     5.7184e-06
6.835	     7.6935e-06
6.84	     8.8075e-06
6.845	     7.61e-06
6.85	     5.1941e-06
6.855	     3.6398e-06
6.86	     2.9205e-06
6.865	     2.1776e-06
6.87	     1.695e-06
6.875	     1.5208e-06
6.88	     1.6597e-06
6.885	     1.9088e-06
6.89	     2.098e-06
6.895	     2.1139e-06
6.9	     2.0422e-06
6.905	     1.9252e-06
6.91	     2.0688e-06
6.915	     2.3779e-06
6.92	     2.4339e-06
6.925	     2.6526e-06
6.93	     3.1827e-06
6.935	     3.6071e-06
6.94	     3.8077e-06
6.945	     3.7555e-06
6.95	     3.4763e-06
6.955	     3.3785e-06
6.96	     3.6272e-06
6.965	     3.4919e-06
6.97	     3.2794e-06
6.975	     2.9768e-06
6.98	     2.9381e-06
6.985	     3.1161e-06
6.99	     2.9028e-06
6.995	     2.389e-06
7	     2.2942e-06
7.005	     2.55e-06
7.01	     3.3541e-06
7.015	     4.293e-06
7.02	     4.6277e-06
7.025	     4.2905e-06
7.03	     4.1068e-06
7.035	     4.1165e-06
7.04	     3.7883e-06
7.045	     3.331e-06
7.05	     2.6644e-06
7.055	     2.2885e-06
7.06	     2.3156e-06
7.065	     2.5747e-06
7.07	     3.0691e-06
7.075	     3.344e-06
7.08	     2.9585e-06
7.085	     3.1086e-06
7.09	     3.2557e-06
7.095	     3.2137e-06
7.1	     3.6552e-06
7.105	     4.1529e-06
7.11	     3.1022e-06
7.115	     2.6255e-06
7.12	     2.7888e-06
7.125	     3.0922e-06
7.13	     3.7359e-06
7.135	     4.9325e-06
7.14	     6.4054e-06
7.145	     6.6959e-06
7.15	     5.3009e-06
7.155	     4.8471e-06
7.16	     4.8438e-06
7.165	     4.6112e-06
7.17	     3.8754e-06
7.175	     3.6501e-06
7.18	     3.361e-06
7.185	     3.3277e-06
7.19	     3.8269e-06
7.195	     4.2692e-06
7.2	     3.9466e-06
7.205	     4.008e-06
7.21	     4.3432e-06
7.215	     4.1468e-06
7.22	     3.6916e-06
7.225	     3.3756e-06
7.23	     3.9062e-06
7.235	     4.8418e-06
7.24	     5.1462e-06
7.245	     4.3715e-06
7.25	     3.6979e-06
7.255	     4.7426e-06
7.26	     7.6445e-06
7.265	     8.4659e-06
7.27	     7.4614e-06
7.275	     6.3417e-06
7.28	     5.8794e-06
7.285	     5.229e-06
7.29	     3.9536e-06
7.295	     3.1702e-06
7.3	     3.0805e-06
7.305	     3.0001e-06
7.31	     3.0737e-06
7.315	     3.4393e-06
7.32	     3.7121e-06
7.325	     3.5731e-06
7.33	     3.0201e-06
7.335	     2.6187e-06
7.34	     2.5893e-06
7.345	     2.8411e-06
7.35	     2.8826e-06
7.355	     2.8275e-06
7.36	     2.7863e-06
7.365	     2.9311e-06
7.37	     3.2023e-06
7.375	     3.4843e-06
7.38	     3.6001e-06
7.385	     3.9337e-06
7.39	     4.9393e-06
7.395	     5.9397e-06
7.4	     6.6921e-06
7.405	     7.3646e-06
7.41	     6.8441e-06
7.415	     6.3524e-06
7.42	     5.9404e-06
7.425	     5.5277e-06
7.43	     5.663e-06
7.435	     5.9845e-06
7.44	     5.3623e-06
7.445	     4.7934e-06
7.45	     4.8357e-06
7.455	     5.5013e-06
7.46	     6.055e-06
7.465	     6.1972e-06
7.47	     6.2359e-06
7.475	     6.5024e-06
7.48	     6.451e-06
7.485	     5.7465e-06
7.49	     5.2611e-06
7.495	     5.1635e-06
7.5	     4.1814e-06
7.505	     3.9885e-06
7.51	     4.7478e-06
7.515	     5.792e-06
7.52	     6.0551e-06
7.525	     4.5308e-06
7.53	     3.405e-06
7.535	     3.1579e-06
7.54	     3.3149e-06
7.545	     3.4626e-06
7.55	     3.6222e-06
7.555	     3.9001e-06
7.56	     4.2578e-06
7.565	     4.3918e-06
7.57	     4.66e-06
7.575	     5.2212e-06
7.58	     5.7379e-06
7.585	     4.9811e-06
7.59	     4.0381e-06
7.595	     4.1327e-06
7.6	     5.2155e-06
7.605	     5.6041e-06
7.61	     5.1098e-06
7.615	     4.5022e-06
7.62	     4.7438e-06
7.625	     5.501e-06
7.63	     5.435e-06
7.635	     6.3881e-06
7.64	     6.5816e-06
7.645	     5.4439e-06
7.65	     4.6956e-06
7.655	     4.4277e-06
7.66	     4.3202e-06
7.665	     4.2233e-06
7.67	     3.8603e-06
7.675	     3.6813e-06
7.68	     3.1533e-06
7.685	     2.6495e-06
7.69	     2.3498e-06
7.695	     2.342e-06
7.7	     2.3134e-06
7.705	     2.6107e-06
7.71	     2.933e-06
7.715	     3.5363e-06
7.72	     4.3537e-06
7.725	     6.0573e-06
7.73	     6.9401e-06
7.735	     7.6633e-06
7.74	     8.5082e-06
7.745	     9.3031e-06
7.75	     9.0892e-06
7.755	     7.2557e-06
7.76	     5.1098e-06
7.765	     3.9542e-06
7.77	     3.5497e-06
7.775	     3.1398e-06
7.78	     2.9995e-06
7.785	     4.0278e-06
7.79	     6.9668e-06
7.795	     1.0636e-05
7.8	     1.0759e-05
7.805	     9.7494e-06
7.81	     1.0773e-05
7.815	     1.3474e-05
7.82	     1.4122e-05
7.825	     1.2709e-05
7.83	     1.0685e-05
7.835	     8.9108e-06
7.84	     8.7901e-06
7.845	     1.0593e-05
7.85	     1.1622e-05
7.855	     1.0046e-05
7.86	     8.154e-06
7.865	     7.0223e-06
7.87	     6.4864e-06
7.875	     5.8484e-06
7.88	     5.6848e-06
7.885	     5.4718e-06
7.89	     5.4809e-06
7.895	     5.5803e-06
7.9	     5.5373e-06
7.905	     5.3981e-06
7.91	     5.0285e-06
7.915	     4.5578e-06
7.92	     3.9368e-06
7.925	     3.349e-06
7.93	     2.9753e-06
7.935	     3.1522e-06
7.94	     4.0285e-06
7.945	     5.2993e-06
7.95	     5.7502e-06
7.955	     5.0942e-06
7.96	     4.3136e-06
7.965	     3.9089e-06
7.97	     3.9861e-06
7.975	     3.8963e-06
7.98	     3.9882e-06
7.985	     4.7885e-06
7.99	     5.0754e-06
7.995	     5.1066e-06
8	     5.6489e-06
8.005	     5.9732e-06
8.01	     6.104e-06
8.015	     6.4248e-06
8.02	     7.1863e-06
8.025	     7.7744e-06
8.03	     7.9381e-06
8.035	     8.3209e-06
8.04	     8.4962e-06
8.045	     8.8807e-06
8.05	     9.4207e-06
8.055	     1.1069e-05
8.06	     1.367e-05
8.065	     1.3535e-05
8.07	     1.1493e-05
8.075	     1.0103e-05
8.08	     8.4257e-06
8.085	     7.7685e-06
8.09	     7.2655e-06
8.095	     7.3825e-06
8.1	     6.3991e-06
8.105	     4.8071e-06
8.11	     3.815e-06
8.115	     3.6569e-06
8.12	     4.0312e-06
8.125	     4.8438e-06
8.13	     5.4443e-06
8.135	     5.9145e-06
8.14	     6.4631e-06
8.145	     6.9586e-06
8.15	     7.2575e-06
8.155	     7.0334e-06
8.16	     6.5571e-06
8.165	     5.6339e-06
8.17	     5.027e-06
8.175	     5.2282e-06
8.18	     6.7181e-06
8.185	     9.5678e-06
8.19	     1.043e-05
8.195	     9.6585e-06
8.2	     8.9744e-06
8.205	     8.9657e-06
8.21	     8.6052e-06
8.215	     7.8765e-06
8.22	     6.945e-06
8.225	     5.54e-06
8.23	     5.379e-06
8.235	     7.8236e-06
8.24	     1.3519e-05
8.245	     1.8186e-05
8.25	     1.734e-05
8.255	     1.4195e-05
8.26	     9.9743e-06
8.265	     7.1859e-06
8.27	     5.7744e-06
8.275	     5.3008e-06
8.28	     4.671e-06
8.285	     5.0335e-06
8.29	     5.931e-06
8.295	     6.2198e-06
8.3	     6.0843e-06
8.305	     5.7162e-06
8.31	     6.0404e-06
8.315	     5.7292e-06
8.32	     4.8695e-06
8.325	     4.7873e-06
8.33	     5.5374e-06
8.335	     8.0653e-06
8.34	     1.167e-05
8.345	     1.24e-05
8.35	     1.3317e-05
8.355	     1.4546e-05
8.36	     1.7393e-05
8.365	     1.7745e-05
8.37	     1.4585e-05
8.375	     1.0256e-05
8.38	     7.1752e-06
8.385	     5.7593e-06
8.39	     6.2379e-06
8.395	     7.3286e-06
8.4	     7.5726e-06
8.405	     8.1077e-06
8.41	     8.4785e-06
8.415	     8.4698e-06
8.42	     8.5113e-06
8.425	     6.8852e-06
8.43	     5.374e-06
8.435	     5.0939e-06
8.44	     5.9823e-06
8.445	     7.1768e-06
8.45	     7.5663e-06
8.455	     8.6915e-06
8.46	     1.1725e-05
8.465	     1.6664e-05
8.47	     1.9274e-05
8.475	     1.8246e-05
8.48	     1.5815e-05
8.485	     1.4274e-05
8.49	     1.142e-05
8.495	     9.7548e-06
8.5	     8.5656e-06
8.505	     8.7035e-06
8.51	     9.3902e-06
8.515	     9.9718e-06
8.52	     9.9276e-06
8.525	     1.0298e-05
8.53	     9.4679e-06
8.535	     8.508e-06
8.54	     7.2763e-06
8.545	     6.5596e-06
8.55	     6.757e-06
8.555	     6.7835e-06
8.56	     6.9166e-06
8.565	     7.628e-06
8.57	     8.0534e-06
8.575	     8.6212e-06
8.58	     8.0553e-06
8.585	     8.6063e-06
8.59	     1.0443e-05
8.595	     1.0551e-05
8.6	     1.296e-05
8.605	     1.8163e-05
8.61	     2.5015e-05
8.615	     3.2308e-05
8.62	     3.5686e-05
8.625	     3.255e-05
8.63	     2.6247e-05
8.635	     1.8864e-05
8.64	     1.5079e-05
8.645	     1.3098e-05
8.65	     1.2857e-05
8.655	     1.2464e-05
8.66	     1.2391e-05
8.665	     1.2655e-05
8.67	     1.2321e-05
8.675	     1.0463e-05
8.68	     8.1592e-06
8.685	     7.3731e-06
8.69	     7.2467e-06
8.695	     7.5021e-06
8.7	     7.2708e-06
8.705	     7.4721e-06
8.71	     8.2927e-06
8.715	     9.9304e-06
8.72	     1.2918e-05
8.725	     1.4304e-05
8.73	     1.5328e-05
8.735	     1.3547e-05
8.74	     1.1922e-05
8.745	     1.047e-05
8.75	     1.0616e-05
8.755	     1.023e-05
8.76	     9.9054e-06
8.765	     9.1996e-06
8.77	     8.7213e-06
8.775	     9.489e-06
8.78	     1.0549e-05
8.785	     1.2029e-05
8.79	     1.2071e-05
8.795	     1.1843e-05
8.8	     1.1892e-05
8.805	     1.1769e-05
8.81	     1.142e-05
8.815	     1.1432e-05
8.82	     1.1309e-05
8.825	     1.2412e-05
8.83	     1.4308e-05
8.835	     1.4363e-05
8.84	     1.3442e-05
8.845	     1.2637e-05
8.85	     1.2019e-05
8.855	     1.1104e-05
8.86	     1.1942e-05
8.865	     1.2611e-05
8.87	     1.4445e-05
8.875	     1.7687e-05
8.88	     2.2566e-05
8.885	     2.2486e-05
8.89	     2.1981e-05
8.895	     2.2889e-05
8.9	     2.6526e-05
8.905	     3.0812e-05
8.91	     2.8972e-05
8.915	     2.6757e-05
8.92	     2.3204e-05
8.925	     2.2915e-05
8.93	     2.3556e-05
8.935	     2.2975e-05
8.94	     2.094e-05
8.945	     1.7172e-05
8.95	     1.4762e-05
8.955	     1.1602e-05
8.96	     1.051e-05
8.965	     9.8922e-06
8.97	     9.8624e-06
8.975	     1.0041e-05
8.98	     1.051e-05
8.985	     1.0962e-05
8.99	     1.1484e-05
8.995	     1.219e-05
9	     1.2128e-05
9.005	     1.1785e-05
9.01	     1.1824e-05
9.015	     1.3182e-05
9.02	     1.7827e-05
9.025	     2.0703e-05
9.03	     1.9493e-05
9.035	     1.8388e-05
9.04	     1.9054e-05
9.045	     1.8509e-05
9.05	     1.8813e-05
9.055	     2.241e-05
9.06	     2.4712e-05
9.065	     2.2957e-05
9.07	     2.1834e-05
9.075	     2.0892e-05
9.08	     1.9925e-05
9.085	     1.6163e-05
9.09	     1.4613e-05
9.095	     1.6536e-05
9.1	     1.9133e-05
9.105	     1.8844e-05
9.11	     1.8133e-05
9.115	     1.9467e-05
9.12	     2.424e-05
9.125	     3.2871e-05
9.13	     3.8467e-05
9.135	     3.7366e-05
9.14	     3.4401e-05
9.145	     2.7915e-05
9.15	     2.2843e-05
9.155	     2.2537e-05
9.16	     2.9111e-05
9.165	     3.6606e-05
9.17	     4.018e-05
9.175	     3.238e-05
9.18	     2.3949e-05
9.185	     1.9517e-05
9.19	     1.9082e-05
9.195	     2.2057e-05
9.2	     2.6608e-05



==> babarsym.tex <==
%%%%%   Standard symbols for use in BABAR papers and BAD Notes
%%%%%
%%%%%   Revised   05/22/01 P. Dauncey     Added \hepex, etc. and clean up a bit
%%%%%   Revised   12/07/00 D. Hitlin      Added features of D. Kirkby's HEP.sty
%%%%%   Revised   07/13/00 R. Waldi       Corrected \Kbar, \Bbar ... macros
%%%%%   Revised   07/13/00 D. MacFarlane  Replaced incorrect \chic1 symbols
%%%%%   Revised   07/05/00 P. Dauncey     Added \mes, \mec, removed \O
%%%%%   Revised   07/04/00 D. MacFarlane  Added scalable version of BABAR
%%%%%   Revised   07/01/00 D. MacFarlane
%%%%%   Revised   06/21/00 D. Hitlin
%%%%%   Original  06/10/00 D. Hitlin
%%%%%   Revision of TDR and Physics Book symbol file
%%%%%

\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% BABAR ... THE NAME OF THE COLLABORATION %%%%

% Huge boldface
\def\hbabar{\mbox{{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A}\hspace{-0.03em}{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A\hspace{-0.03em}R}}}
% LARGE
\def\Lbabar{\mbox{{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A}\hspace{-0.07em}{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A\hspace{-0.02em}R}}}
% Large
\def\lbabar{\mbox{{\large\sl B}\hspace{-0.4em} {\normalsize\sl A}\hspace{-0.03em}{\large\sl B}\hspace{-0.4em} {\normalsize\sl A\hspace{-0.02em}R}}}
% normal size
%\def\babar{\mbox{\sl B\hspace{-0.4em} {\small\sl A}\hspace{-0.37em} \sl B\hspace{-0.4em} {\small\sl A\hspace{-0.02em}R}}}
% replace normalsize with scalable version       dbm 7/4/00
\usepackage{relsize}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}

% Obsolete
\newcommand{\dstr}{\ensuremath{\Dstar}\xspace}
\newcommand{\dstrstr}{\ensuremath{D^{**}}\xspace}
\newcommand{\dsp}{\ensuremath{\Dstarp}\xspace}
\newcommand{\dsm}{\ensuremath{\Dstarm}\xspace}
\newcommand{\dsz}{\ensuremath{\Dstarz}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}

% added by GHM on March 25, 2003 -- from Andrei Gritsan
\def\BorBbar    {\kern 0.18em\optbar{\kern -0.18em B}{}\xspace}
\def\DorDbar    {\kern 0.18em\optbar{\kern -0.18em D}{}\xspace}
\def\KorKbar    {\kern 0.18em\optbar{\kern -0.18em K}{}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}

%\def\chic1{\ensuremath{\chi_{c1}}}
%\def\chic2{\ensuremath{\chi_{c2}}}
%\def\chic3{\ensuremath{\chi_{c3}}}
\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} % dbm


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% TAU BRANCHING FRACTIONS %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\BR         {{\ensuremath{\cal B}\xspace}}
\def\BRtauptoe  {\ensuremath{\BR(\taup \to \ep)}\xspace}
\def\BRtaumtoe  {\ensuremath{\BR(\taum \to \en)}\xspace}
\def\BRtauptomu {\ensuremath{\BR(\taup \to \mup)}\xspace}
\def\BRtaumtomu {\ensuremath{\BR(\taum \to \mun)}\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  LIGHT HADRON DECAYS %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etaprepp}{\ensuremath{\etapr \to \eta \pipi}\xspace}
\newcommand{\etaprrg} {\ensuremath{\etapr \to \rho^0 \g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  B DECAYS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\bpsiks     {\ensuremath{\Bz \to \jpsi \KS}\xspace}
\def\bpsikst    {\ensuremath{\Bz \to \jpsi \Kstar}\xspace}
\def\bpsikl     {\ensuremath{\Bz \to \jpsi \KL}\xspace}
\def\bpsikzeropi{\ensuremath{\Bz \to \jpsi \Kstarz (\to \KL \piz)}\xspace}
\def\bpsikpluspi{\ensuremath{\Bu \to \jpsi \Kstarp (\to \KL \pip)}\xspace}
\def\bpsikpi    {\ensuremath{\Bz/\Bzb \to \jpsi (\to \mumu) \Kpm \pimp}\xspace}
\def\bupsik     {\ensuremath{\Bpm \to \jpsi (\to \mumu) \Kpm}\xspace}
\def\bpsiX      {\ensuremath{\Bz \to \jpsi \X}\xspace}

\def\Bzbtomu    {\ensuremath{\Bzb \to \mu \X}\xspace}
\def\Bzbtox     {\ensuremath{\Bzb \to \X}\xspace}
\def\Bztopipi   {\ensuremath{\Bz \to \pipi}\xspace}
\def\Bztokpi    {\ensuremath{\Bz \to \Kpm \pimp}\xspace}
\def\Bztorhopi  {\ensuremath{\Bz \to \rho^+ \pim}\xspace}
\def\Bztorhorho {\ensuremath{\Bz \to \rho \rho}\xspace}
\def\Bztokrho   {\ensuremath{\Bz \to K \rho}\xspace}
\def\Bztokstpi  {\ensuremath{\Bz \to \Kstar \pi}\xspace}
\def\Bztoapi    {\ensuremath{\Bz \to a_1 \pi}\xspace}
\def\Bztodd     {\ensuremath{\Bz \to \DpDm}\xspace}
\def\Bztodstd   {\ensuremath{\Bz \to \Dstarp \Dm}\xspace}
\def\Bztodstdst {\ensuremath{\Bz \to \Dstarp \Dstarm}\xspace}

\def\BtoDK      {\ensuremath{B \to DK}\xspace}
\def\Btodstlnu  {\ensuremath{B \to \Dstar \ell \nu}\xspace}
\def\Btodstdlnu {\ensuremath{B \to \Dstar(D) \ell \nu}\xspace}
\def\Btorholnu  {\ensuremath{B \to \rho \ell \nu}\xspace}
\def\Btopilnu   {\ensuremath{B \to \pi \ell \nu}\xspace}

\def\Btoetah    {\ensuremath{B \to \eta h}\xspace}
\def\Btoetaph   {\ensuremath{B \to \etapr h}\xspace}

\newcommand{\Betaprks}{\ensuremath{\Bz \to \etapr \KS}\xspace}
\newcommand{\Betaprkz}{\ensuremath{\Bz \to \etapr \Kz}\xspace}

\def\btosgam    {\ensuremath{b \to s \g}\xspace}
\def\btodgam    {\ensuremath{b \to d \g}\xspace}
\def\btosll     {\ensuremath{b \to s \ellell}\xspace}
\def\btosnunu   {\ensuremath{b \to s \nunub}\xspace}
\def\btosgaga   {\ensuremath{b \to s \gaga}\xspace}
\def\btosglue   {\ensuremath{b \to s g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  Y(4S) DECAYS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\upsbb   {\ensuremath{\FourS \to \BB}\xspace}
\def\upsbzbz {\ensuremath{\FourS \to \BzBzb}\xspace}
\def\upsbpbm {\ensuremath{\FourS \to \BpBm}\xspace}
\def\upspsikl{\ensuremath{\FourS \to (\bpsikl) (\Bzbtox)}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  TAU DECAYS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\tauptoe    {\ensuremath{\taup \to \ep \nunub}\xspace}
\def\taumtoe    {\ensuremath{\taum \to \en \nunub}\xspace}
\def\tauptomu   {\ensuremath{\taup \to \mup \nunub}\xspace}
\def\taumtomu   {\ensuremath{\taum \to \mun \nunub}\xspace}
\def\tauptopi   {\ensuremath{\taup \to \pip \nub}\xspace}
\def\taumtopi   {\ensuremath{\taum \to \pim \nu}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% GAMMA-GAMMA REACTIONS %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ggtopi     {\ensuremath{\gaga \to \pipi}\xspace}
\def\ggtopiz    {\ensuremath{\gaga \to \ppz}\xspace}
\def\ggstox     {\ensuremath{\ggstar \to \X(1420) \to \kaon \kaon \pi}\xspace}
\def\ggstoeta   {\ensuremath{\ggstar \to \eta(550) \to \pipi \piz}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   KINEMATICS    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{$p$}\xspace}
%\def\pxy        {\mbox{$p_{\rm t}$}
\def\pxy        {\mbox{$p_T$}\xspace}
%\def\pt         {\mbox{$p_{\rm t}$}\xspace}
\def\pt         {\mbox{$p_T$}\xspace}
\def\mes        {\mbox{$m_{\rm ES}$}\xspace}
\def\mec        {\mbox{$m_{\rm EC}$}\xspace}
\def\DeltaE     {\mbox{$\Delta E$}\xspace}

\def\pbcm {\ensuremath{p^*_{\Bz}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   GEOMETRY    %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mphi       {\mbox{$\phi$}\xspace}
\def\mtheta     {\mbox{$\theta$}\xspace}
\def\ctheta     {\mbox{$\cos\theta$}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}
%\def\ev   {\ensuremath{\rm \,e\kern -0.08em V}}
%\def\kev  {\ensuremath{\rm \,ke\kern -0.08em V}} 
%\def\mev  {\ensuremath{\rm \,Me\kern -0.08em V}} 
%\def\gev  {\ensuremath{\rm \,Ge\kern -0.08em V}} 
%\def\gevc {\ensuremath{\rm \,Ge\kern -0.08em V\!/c}} 
%\def\gevc {\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c}} 
%\def\tev  {\ensuremath{\rm \,Te\kern -0.08em V}}
%\def\mevc {\ensuremath{\rm \,Me\kern -0.08em V\!/c}} 
%\def\mevc {\ensuremath{{\rm \,Me\kern -0.08em V\!/}c}} 
%\def\gevcc{\ensuremath{\rm \,Ge\kern -0.08em V\!/c^2}} 
%\def\mevcc{\ensuremath{\rm \,Me\kern -0.08em V\!/c^2}} 
%\def\gevcc{\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c^2}} 
%\def\mevcc{\ensuremath{{\rm \,Me\kern -0.08em V\!/}c^2}} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
%\def\mum  {\ensuremath{{\rm \,\mum}}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter 
%\def\muma {\ensuremath{\rm \,\mum}^2\xspace}
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

%%\def\s{\ensuremath{\rm {\,s}}} %% second - this displays nothing  - why?
\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second - this works - jw 4/19
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees


%\def\m          {\ensuremath{\rm \,m}}    %% meter
%\def\ma         {\ensuremath{\rm \,m}^2}  %% meter squared
%\def\cm         {\ensuremath{\rm \,cm}}   %% centimeter
%\def\cma        {\ensuremath{\rm \,cm}^2} %% centimeter squared
\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}
%\def\mm         {\ensuremath{\rm \,mm}}   %% millimeter
%\def\mma        {\ensuremath{\rm \,mm}^2} %% millimeter squared
%\def\mum        {\ensuremath{\,\mu\rm m}} %% mu meter
%\def\muma       {\ensuremath{\,\mu\rm m^2}}


\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    

%\renewcommand{\bar}[1]{\overline{#1}}  

% Some more (from Helen)
%\def\O{{\ensuremath{\cal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
%\def\S{{\ensuremath{\cal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}


\def\pep2{PEP-II}
\def\BF{$B$ Factory}
\def\abf {asymmetric \BF}
\def\sx    {\ensuremath{\sigma_x}\xspace}     
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}


\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}


% Data processing
\def\kbytes     {\ensuremath{{\rm \,kbytes}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbytes/s}}\xspace}
\def\kbits      {\ensuremath{{\rm \,kbits}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbits/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbits/s}}\xspace}
\def\mbytes     {\ensuremath{{\rm \,Mbytes}}\xspace}
\def\mbps       {\ensuremath{{\rm \,Mbyte/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbytes/s}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbits/s}}\xspace}
\def\gbytes     {\ensuremath{{\rm \,Gbytes}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbytes/s}}\xspace}
\def\tbytes     {\ensuremath{{\rm \,Tbytes}}\xspace}
\def\tbpy       {\ensuremath{{\rm \,Tbytes/yr}}\xspace}
%




% QCD parameters

\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\LMSb}{%
  \ensuremath{\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}\xspace
}

% Electroweak parameters

\newcommand{\tw}{\ensuremath{\theta_{\scriptscriptstyle W}}\xspace}
\newcommand{\twb}{%
  \ensuremath{\overline{\theta}_{\scriptscriptstyle W}}\xspace
}
\newcommand{\Afb}[1]{{\ensuremath{A_{\scriptscriptstyle FB}^{#1}}}\xspace}
\newcommand{\gv}[1]{{\ensuremath{g_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\ga}[1]{{\ensuremath{g_{\scriptscriptstyle A}^{#1}}}\xspace}
\newcommand{\gvb}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\gab}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle A}^{#1}}}\xspace}


% CKM, CP violation

\def\eps{\varepsilon\xspace}
\def\epsK{\varepsilon_K\xspace}
\def\epsB{\varepsilon_B\xspace}
\def\epsp{\varepsilon^\prime_K\xspace}

\def\CP                {\ensuremath{C\!P}\xspace}
%\def\CPT               {\ensuremath{C\!P\!T}\xspace}
\def\CPT               {\ensuremath{C\!PT}\xspace} % Looks better without \!
% added by GHM on March 25, 2003
\def\C       {\ensuremath{C}\xspace}
\def\P       {\ensuremath{P}\xspace}
\def\T       {\ensuremath{T}\xspace}



\def\epstag  {\ensuremath{\varepsilon_{\rm tag}}\xspace}
\def\tagfac  {\ensuremath{\epstag(1-2w)^2}\xspace}

\def\rhobar {\ensuremath{\overline \rho}\xspace}
\def\etabar {\ensuremath{\overline \eta}\xspace}
%\def\paramest {\ensuremath{{\hat A}, {\hat \rho}, {\hat \eta} }}
%\def\ssparamest {\ensuremath{{\hat A}, {\hat {\sin 2 \alpha}}, 
%{\hat {\sin 2 \beta}} }}
\def\meas {\ensuremath{|V_{cb}|, |\frac{V_{ub}}{V_{cb}}|, 
|\varepsilon_K|, \Delta m_{B_d}}\xspace}

\def\Vud  {\ensuremath{|V_{ud}|}\xspace}
\def\Vcd  {\ensuremath{|V_{cd}|}\xspace}
\def\Vtd  {\ensuremath{|V_{td}|}\xspace}
\def\Vus  {\ensuremath{|V_{us}|}\xspace}
\def\Vcs  {\ensuremath{|V_{cs}|}\xspace}
\def\Vts  {\ensuremath{|V_{ts}|}\xspace}
\def\Vub  {\ensuremath{|V_{ub}|}\xspace}
\def\Vcb  {\ensuremath{|V_{cb}|}\xspace}
\def\Vtb  {\ensuremath{|V_{tb}|}\xspace}

%\def\sa{${\sin\! 2 \alpha  }$\xspace}
%\def\sb{${\sin\! 2 \beta   }$\xspace}
%\def\sg{${\sin\! 2 \gamma  }$\xspace}

% added by Gautier for tagging, tagmix, and sin2beta
\def\stwoa{\ensuremath{\sin\! 2 \alpha  }\xspace}
\def\stwob{\ensuremath{\sin\! 2 \beta   }\xspace}
\def\stwog{\ensuremath{\sin\! 2 \gamma  }\xspace}
\def\mistag{\ensuremath{w}\xspace}
\def\dilution{\ensuremath{\cal D}\xspace}
\def\deltaz{\ensuremath{{\rm \Delta}z}\xspace}
\def\deltat{\ensuremath{{\rm \Delta}t}\xspace}
\def\deltamd{\ensuremath{{\rm \Delta}m_d}\xspace}

\newcommand{\fsubd}{\ensuremath{f_D}}\xspace
\newcommand{\fds}{\ensuremath{f_{D_s}}\xspace}
\newcommand{\fsubb}{\ensuremath{f_B}\xspace}
\newcommand{\fbd}{\ensuremath{f_{B_d}}\xspace}
\newcommand{\fbs}{\ensuremath{f_{B_s}}\xspace}
\newcommand{\bsubb}{\ensuremath{B_B}\xspace}
\newcommand{\bbd}{\ensuremath{B_{B_d}}\xspace}
\newcommand{\bbs}{\ensuremath{B_{B_s}}\xspace}
\newcommand{\rgbb}{\ensuremath{\hat{B}_B}\xspace}
\newcommand{\rgbbd}{\ensuremath{\hat{B}_{B_d}}\xspace}
\newcommand{\rgbbs}{\ensuremath{\hat{B}_{B_s}}\xspace}
\newcommand{\rgbk}{\ensuremath{\hat{B}_K}\xspace}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace}

%\newcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}




% Journal References

% These bases are useful for ``submitted to'' when no volume is needed
\newcommand{\epjBase}        {Eur.\ Phys.\ Jour.\xspace}
\newcommand{\jprlBase}       {Phys.\ Rev.\ Lett.\xspace}
\newcommand{\jprBase}        {Phys.\ Rev.\xspace}
\newcommand{\jplBase}        {Phys.\ Lett.\xspace}
%\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Meth.\xspace}
%\newcommand{\nimBaseB}       {Nucl.\ Instr.\ and Meth.\xspace}
%\newcommand{\nimBaseC}       {Nucl.\ Instr.\ and Methods\xspace}
%\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods\xspace}
%\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Meth.\xspace}
% update the following based on input from John Ripka, Asst. Editor at PRL, August 2006
\newcommand{\nimBaseA}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ A\xspace}
\newcommand{\nimBaseB}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ B\xspace}
\newcommand{\nimBaseC}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ C\xspace}
\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ D\xspace}
\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ E\xspace}
\newcommand{\npBase}         {Nucl.\ Phys.\xspace}
\newcommand{\zpBase}         {Z.\ Phys.\xspace}


\newcommand{\apas}      [1]  {{Acta Phys.\ Austr.\ Suppl.\ {\bf #1}}}
\newcommand{\app}       [1]  {{Acta Phys.\ Polon.\ {\bf #1}}}
\newcommand{\ace}       [1]  {{Adv.\ Cry.\ Eng.\ {\bf #1}}}
\newcommand{\anp}       [1]  {{Adv.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\annp}      [1]  {{Ann.\ Phys.\ {\bf #1}}}
\newcommand{\araa}      [1]  {{Ann.\ Rev.\ Astr.\ Ap.\ {\bf #1}}}
\newcommand{\arnps}     [1]  {{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\bf #1}}}
\newcommand{\arns}      [1]  {{Ann.\ Rev.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\appopt}    [1]  {{Appl.\ Opt.\ {\bf #1}}}
\newcommand{\japj}      [1]  {{Astro.\ Phys.\ J.\ {\bf #1}}}
\newcommand{\baps}      [1]  {{Bull.\ Am.\ Phys.\ Soc.\ {\bf #1}}}
\newcommand{\seis}      [1]  {{Bull.\ Seismological Soc.\ of Am.\ {\bf #1}}}
\newcommand{\cmp}       [1]  {{Commun.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\cnpp}      [1]  {{Comm.\ Nucl.\ Part.\ Phys.\ {\bf #1}}}
\newcommand{\cpc}       [1]  {{Comput.\ Phys.\ Commun.\ {\bf #1}}}
\newcommand{\epj}       [1]  {\epjBase\ {\bf #1}}
%\newcommand{\epjc}      [1]  {{Eur.\ Phys.\ Jour.\ C~{\bf #1}}}
\newcommand{\epjc}      [1]  {\epjBase\ C~{\bf #1}}
\newcommand{\fizika}    [1]  {{Fizika~{\bf #1}}}
\newcommand{\fp}        [1]  {{Fortschr.\ Phys.\ {\bf #1}}}
\newcommand{\ited}      [1]  {{IEEE Trans.\ Electron.\ Devices~{\bf #1}}}
\newcommand{\itns}      [1]  {{IEEE Trans.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\ijqe}      [1]  {{IEEE J.\ Quantum Electron.\ {\bf #1}}}
\newcommand{\ijmp}      [1]  {{Int.\ Jour.\ Mod.\ Phys.\ {\bf #1}}}
\newcommand{\ijmpa}     [1]  {{Int.\ J.\ Mod.\ Phys.\ {\bf A{\bf #1}}}}
\newcommand{\jl}        [1]  {{JETP Lett.\ {\bf #1}}}
\newcommand{\jetp}      [1]  {{JETP~{\bf #1}}}
\newcommand{\jpg}       [1]  {{J.\ Phys.\ {\bf G{\bf #1}}}}
\newcommand{\jap}       [1]  {{J.\ Appl.\ Phys.\ {\bf #1}}}
\newcommand{\jmp}       [1]  {{J.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\jmes}      [1]  {{J.\ Micro.\ Elec.\ Sys.\ {\bf #1}}}
%\newcommand{\josa}      [1]  {{J.\ Opt.\ Soc.\ Am.\ {\bf #1}}}
\newcommand{\mpl}       [1]  {{Mod.\ Phys.\ Lett.\ {\bf #1}}}

%\newcommand{\nim}       [1]  {{Nucl.\ Instrum.\ and Methods~{\bf #1}}}
\newcommand{\nim}       [1]  {\nimBaseC~{\bf #1}}
\newcommand{\nimaa}       [1]  {\nimBaseE~{\bf #1}}
%\newcommand{\nima}      [1]  {{Nucl.\ Instrum.\ Methods~{\bf A{\bf #1}}}}
\newcommand{\nima}      [1]  {\nimBaseA~{\bf #1}}
\newcommand{\nimb}      [1]  {\nimBaseB~{\bf #1}}
\newcommand{\nimc}      [1]  {\nimBaseC~{\bf #1}}
\newcommand{\nimd}      [1]  {\nimBaseD~{\bf #1}}
\newcommand{\nime}      [1]  {\nimBaseE~{\bf #1}}
% add commands for NIM articles from earlier periods
% for NIM articles from 1981-1983
\newcommand{\oldnim}    [1]  {Nucl.\ Instrum.\ Methods Phys.\ Res.~{\bf #1}}
% for NIM articles prior to 1981
\newcommand{\oldernim}  [1]  {Nucl.\ Instrum.\ Methods~{\bf #1}}

%\newcommand{\np}        [1]  {{Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\np}        [1]  {\npBase\ {\bf #1}}
%\newcommand{\npb}       [1]  {{Nucl.\ Phys.\ {\bf B{\bf #1}}}}
\newcommand{\npb}       [1]  {\npBase\ B~{\bf #1}}
\newcommand{\npps}      [1]  {{Nucl.\ Phys.\ Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npaps}     [1]  {{Nucl.\ Phys.\ A~Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B~Proc.\ Suppl.\ {\bf #1}}}

\newcommand{\ncim}      [1]  {{Nuo.\ Cim.\ {\bf #1}}}
\newcommand{\optl}      [1]  {{Opt.\ Lett.\ {\bf #1}}}
\newcommand{\optcom}    [1]  {{Opt.\ Commun.\ {\bf #1}}}
\newcommand{\partacc}   [1]  {{Particle Acclerators~{\bf #1}}}
\newcommand{\pan}       [1]  {{Phys.\ Atom.\ Nuclei~{\bf #1}}}
\newcommand{\pflu}      [1]  {{Physics of Fluids~{\bf #1}}}
\newcommand{\ptoday}    [1]  {{Physics Today~{\bf #1}}}

%\newcommand{\jpl}       [1]  {{Phys.\ Lett.\ {\bf #1}}}      % dbm
\newcommand{\jpl}       [1]  {\jplBase\ {\bf #1}}
%\newcommand{\plb}       [1]  {{Phys.\ Lett.\ B~{\bf #1}}}   % dbm
\newcommand{\plb}       [1]  {\jplBase\ B~{\bf #1}}
\newcommand{\prep}      [1]  {{Phys.\ Rep.\ {\bf #1}}}
%\newcommand{\jprl}      [1]  {{Phys.\ Rev.\ Lett.\ {\bf #1}}} % dbm
\newcommand{\jprl}      [1]  {\jprlBase\ {\bf #1}}
%\newcommand{\pr}        [1]  {{Phys.\ Rev.\ {\bf #1}}}
\newcommand{\pr}        [1]  {\jprBase\ {\bf #1}}
%\newcommand{\jpra}      [1]  {{Phys.\ Rev.\ A~{\bf #1}}}
\newcommand{\jpra}      [1]  {\jprBase\ A~{\bf #1}}
%\newcommand{\jprd}      [1]  {{Phys.\ Rev.\ D~{\bf #1}}}
\newcommand{\jprd}      [1]  {\jprBase\ D~{\bf #1}}
%\newcommand{\jpre}      [1]  {{Phys.\ Rev.\ E~{\bf #1}}}
\newcommand{\jpre}      [1]  {\jprBase\ E~{\bf #1}}

\newcommand{\prsl}      [1]  {{Proc.\ Roy.\ Soc.\ Lond.\ {\bf #1}}}
\newcommand{\ppnp}      [1]  {{Prog.\ Part.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\progtp}    [1]  {{Prog.\ Theor.\ Phys.\ {\bf #1}}}
\newcommand{\rpp}       [1]  {{Rep.\ Prog.\ Phys.\ {\bf #1}}}
\newcommand{\jrmp}      [1]  {{Rev.\ Mod.\ Phys.\ {\bf #1}}}  % dbm
\newcommand{\rsi}       [1]  {{Rev.\ Sci.\ Instr.\ {\bf #1}}}
\newcommand{\sci}       [1]  {{Science~{\bf #1}}}
\newcommand{\sjnp}      [1]  {{Sov.\ J.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\spd}       [1]  {{Sov.\ Phys.\ Dokl.\ {\bf #1}}}
\newcommand{\spu}       [1]  {{Sov.\ Phys.\ Usp.\ {\bf #1}}}
\newcommand{\tmf}       [1]  {{Teor.\ Mat.\ Fiz.\ {\bf #1}}}
\newcommand{\yf}        [1]  {{Yad.\ Fiz.\ {\bf #1}}}
%\newcommand{\zp}        [1]  {{Z.\ Phys.\ {\bf #1}}}
\newcommand{\zp}        [1]  {\zpBase\ {\bf #1}}
%\newcommand{\zpc}       [1]  {{Z.\ Phys.\ C~{\bf #1}}}
\newcommand{\zpc}       [1]  {\zpBase\ C~{\bf #1}}
\newcommand{\zpr}       [1]  {{ZhETF Pis.\ Red.\ {\bf #1}}}

\newcommand{\hepex}     [1]  {hep-ex/{#1}}
\newcommand{\hepph}     [1]  {hep-ph/{#1}}
\newcommand{\hepth}     [1]  {hep-th/{#1}}


%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aslund     {\mbox{\tt Aslund}\xspace}
\def\bbsim      {\mbox{\tt BBsim}\xspace}
\def\beast      {\mbox{\tt Beast}\xspace}
\def\beget      {\mbox{\tt Beget}\xspace}
\def\Bta        {\mbox{\tt Beta}\xspace}
\def\betakfit   {\mbox{\tt BetaKfit}\xspace}
\def\cornelius  {\mbox{\tt Cornelius}\xspace}
\def\evtgen     {\mbox{\tt EvtGen}\xspace}
\def\euclid     {\mbox{\tt Euclid}\xspace}
\def\fitver     {\mbox{\tt FitVer}\xspace}
\def\fluka      {\mbox{\tt Fluka}\xspace}
\def\fortran    {\mbox{\tt Fortran}\xspace}
\def\gcalor     {\mbox{\tt GCalor}\xspace}
\def\geant      {\mbox{\tt GEANT}\xspace}
\def\gheisha    {\mbox{\tt Gheisha}\xspace}
\def\hemicosm   {\mbox{\tt HemiCosm}\xspace}
\def\hepevt     {\mbox{\tt{/HepEvt/}}\xspace}
\def\jetset74   {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}\xspace}
%\def\jetset     {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\mbox{\tt KoralB}\xspace}
\def\minuit     {\mbox{\tt Minuit}\xspace}
\def\objegs     {\mbox{\tt Objegs}\xspace}
\def\paw        {\mbox{\tt Paw}\xspace}
\def\Root       {\mbox{\tt Root}\xspace}
\def\squaw      {\mbox{\tt Squaw}\xspace}
\def\stdhep     {\mbox{\tt StdHep}\xspace}
\def\trackerr   {\mbox{\tt TrackErr}\xspace}
\def\turtle     {\mbox{\tt Decay~Turtle}\xspace}

